Inference-Time Diffusion Model Distillation

Diffusion distillation models effectively accelerate reverse sampling by compressing the process into fewer steps. However, these models still exhibit a performance gap compared to their pre-trained diffusion model counterparts, exacerbated by distribution shifts and accumulated errors during multi-step sampling. To address this, we introduce Distillation++, a novel inference-time distillation framework that reduces this gap by incorporating teacher-guided refinement during sampling. Inspired by recent advances in conditional sampling, our approach recasts student model sampling as a proximal optimization problem with a score distillation sampling loss (SDS). To this end, we integrate distillation optimization during reverse sampling, which can be viewed as teacher guidance that drives student sampling trajectory towards the clean manifold using pre-trained diffusion models. Thus, Distillation++ improves the denoising process in real-time without additional source data or fine-tuning. Distillation++ demonstrates substantial improvements over state-of-the-art distillation baselines, particularly in early sampling stages, positioning itself as a robust guided sampling process crafted for diffusion distillation models. Code: https://github.com/geonyeong-park/inference_distillation.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/X_suppl_old.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary
%\renewcommand{\thesection}{A{section}}

The supplementary sections are organized as follows. 
Section \ref{sec: pseudocode} introduces the pseudo training algorithm behind our inference-time diffusion distillation framework.
In Section \ref{sec: exp setting}, we provide experimental details. Section \ref{sec: additional results} features additional results. Following this, we delve into the future directions and limitations of the proposed method in Section \ref{sec: discussion}. Code will be released in \url{https://github.com/anony-distillationpp/distillation_pp}.
\vspace{-0.1cm}

\section{Pseudo-code}
\vspace{-0.3cm}
\label{sec: pseudocode}
% 
\begin{algorithm}
\label{pseudocode}
	\caption{Inference-time Diffusion model distillation} 
	\begin{algorithmic}[1]
	    \State {\bfseries Input:} Student model \textcolor{student}{$\theta$}, Teacher model \textcolor{teacher}{$\psi$}, $N$ sampling steps, $k$ number of steps of teacher guidance, CFG scale $\omega$, Teacher guidance scale $\lambda$.
        
        \State {\bfseries Output:} Improved generation $\x_0^*$. \\
        \State $\x_T \sim \Nc(\x_T| 0, I), \quad \triangle t = T / N$
        
            \For {$t=T$ \textbf{to} $\triangle t$}
                \State \textbf{Stage 1.} \textit{Initial student estimation}
                \State $\tweediecstudent(t) = \frac{\x_t - \sqrt{1-\alphabar_t} \epshatstudent(\x_t, \c)}{\sqrt{\alphabar_t}}$
                % \State Sample a set of Gaussian noise $\epsilonb_t^{1:N}$, where the $n$-th noise \(\epsilonb_t^n \in \mathbb{R}^d \sim \Nc(0, I)\).
                \\
                \State \textbf{Stage 2.} \textit{Revised teacher estimation}
                 \If {$\text{step} < k$}
                    \State Renoising step $s = t - \triangle t$.
                    \State $\x_s = \sqrt{\alphabar_s} \tweediecstudent(t) + \sqrt{1-\alphabar_s} \epsilonb.$ ($\epsilonb \sim \Nc(\epsilonb| 0, I))$
                    \State $\tweediecteacher(s) = \frac{\x_s - \sqrt{1-\alphabar_s} \epshatteacher(\x_s, \c)}{\sqrt{\alphabar_s}}$.
                    \State $\tweedieppc(t) = (1-\lambda) \tweediecstudent(t) + \lambda \tweediecteacher(s)$
                \Else
                    \State $\tweedieppc(t) = \tweediecstudent(t)$
                \EndIf
                \State Update $\x_{t-\triangle t}$ by forwarding $\tweedieppc(t)$. 
            \EndFor
             
	\end{algorithmic} 
\end{algorithm}

We fix typo in \eqref{eq: cfg tweedie} with $\tilde{\x}_t \rightarrow \x_t$. 
Also, we note that $k=1$ used in every quantitative analysis, ensuring computational efficiency.
As the proposed framework revises estimation by interpolation, it can be seamlessly extended with a convex combination of multiple teacher revisions. Moreover, as Algorithm 1 is described with random renoising strategy (Line 12), it is fully compatible with general student models ranging from ones directly predicting the PF-ODE endpoint to the progressive distillation branches. 

\section{Experimental details}
\label{sec: exp setting}
\subsection{Extension to other solvers}
For completeness, we extend Distillation++ to accommodate a broader range of ODE/SDE solvers. The core principle lies in steering the \textit{denoising} process with teacher models. Specifically, we consider solving the variance-exploding (VE) PF-ODE, commonly employed in standard diffusion model implementations\footnote{\url{https://github.com/crowsonkb/k-diffusion}}, which can be readily derived via reparameterization of VP diffusion models. Following the notation in \citet{lu2022dpmpp}, we consider a sequence of timesteps $\{t_i\}_{i=0}^M$, where $t_0 = T$ denotes the initial starting point of the reverse sampling (i.e. Gaussian noise).

\textbf{Euler \cite{karras2022elucidating}.} This is in line with DDIM \cite{song2020denoising} and thus included for completeness:
\begin{align*}
    \x_{t_{i+1}} &= \tweedieppc(\x_{t_i}) + \frac{\x_{t_i} - \tweediecstudent(\x_{t_i})}{\sigma_{t_i}}\cdot \sigma_{t_{i+1}},
    \vspace{-0.1cm}
\end{align*}
where $\tweedieppc(\x_{t_i})$ refers to the revised estimate by interpolation. CFG++ \cite{chung2024cfg++} can be integrated by replacing $\tweediecstudent(\x_{t_i})$ with $\textcolor{student}{\hat{\x}_\varnothing^\theta}(\x_{t_i})$.

\textbf{Euler Ancestral.} 
The Euler Ancestral sampler extends the Euler method by introducing stochasticity, taking larger steps and adding a small random noise. This may potentially improve sampling diversity:
\begin{align*}
    \x_{t_{i+1}} &= \tweedieppc(\x_{t_i}) + \frac{\x_{t_i} - \tweediecstudent(\x_{t_i})}{\sigma_{t_i}}\cdot (\sigma_{t_{d_i}} - \sigma_{t_i}) + \sigma_{t_i} \epsilonb,
\end{align*}
where $t_i > t_{d_i} > t_{i+1}$ and $\epsilonb \sim \Nc(\epsilonb| 0, I)$.

\textbf{DPM-solver++ 2M \cite{lu2022dpmpp}.} While many student models support only first-order solvers, customized distillation models in the open-source community\footnote{\url{https://civitai.com/}} are compatible with higher-order solvers like DPM-Solver++ 2M. Using an iterative process initialized with Gaussian noise, DPM-solver++ refines the sampling trajectory with higher-order corrections, enabling precise updates. Similarly as DPM-solver++ 2S, define $\sigma_t := e^{-t},\,h_i := t_i - t_{i-1},$ and $r_i := h_{i-1}/h_{i}$. Given $\x_{t_0}$ initialized as Gaussian noise, the first iteration reads:
\begin{align*}
    \x_{t_1} &= \tweediecstudent(\x_{t_0}) + e^{-h_1}(\x_{t_0} - \tweediecstudent(\x_{t_0})). 
\end{align*}

Then, the following provides higher-order correction:
\begin{align}
\label{eq:dpmpp_2m_cfg_1}
    \bm{D}_i &= \tweediecstudent(\x_{t_{i-1}}) + \frac{1}{2r_i}\left(
    \tweediecstudent(\x_{t_{i-1}}) - \tweediecstudent(\x_{t_{i-2}})
    \right),\\
    \x_{t_i} &= e^{-h_i}\x_{t_{i-1}} - (e^{-h_i} - 1)\bm{D}_i.
\label{eq:dpmpp_2m_cfg_2}
\end{align}

Rearranging \eqref{eq:dpmpp_2m_cfg_1}, \eqref{eq:dpmpp_2m_cfg_2}, we can rewrite the update steps as
\begin{align}
\label{eq:dpmpp_2m_cfg_rearrange}
    \x_{t_i} &= \tweediecstudent(\x_{t_{i-1}}) - e^{-h_i}\tweediecstudent(\x_{t_{i-1}}) \nonumber \\
    &+ \frac{1 - e^{-h_i}}{2r_i}\left(
    \tweediecstudent(\x_{t_{i-1}}) - \tweediecstudent(\x_{t_{i-2}})
    \right) + e^{-h_i}\x_{t_{i-1}}. \nonumber
\end{align}

As we are interested in modulating the final form of denoised estimates, Distillation++ can be applied as follows:
\begin{align}
    \x_{t_i} &= \tweedieppc(\x_{t_{i-1}}) - e^{-h_i}\tweediecstudent(\x_{t_{i-1}}) \nonumber \\
    &+ \frac{1 - e^{-h_i}}{2r_i}\left(
    \tweediecstudent(\x_{t_{i-1}}) - \tweediecstudent(\x_{t_{i-2}})
    \right) + e^{-h_i}\x_{t_{i-1}}. \nonumber
\end{align}
% deterministic score: 어느정도 학습된 trajectory를 따라 보낼 수 있기 때문에, 적은 NFE 상에서 더 효과적일 수도 있다. 

Ancestral variants (DPM-solver++ 2M A) can be readily derived by similarly adding a random noise.

\subsection{Experiment Setup}

In this work, we employ several diffusion distillation models: DMD2 \cite{yin2024improved}, SDXL-Turbo \cite{sauer2023adversarial}, SDXL-Lightning \cite{lin2024sdxl}, LCM \cite{luo2023latent}, LCM-LoRA \cite{luo2023lcmlora}, and SDXL-Lightning LoRA. These models rely on classifier-free guidance (CFG) with a fixed guidance scale during training. We use $w=7.5$ for CFG with teacher models $\tweediecteacher(s)$.

Baselines using 4 sampling steps include SDXL-Lightning, DMD2, and SDXL-Turbo, while LCM and LCM-LoRA use 8 sampling steps. Specifically, for Table \ref{table: result}, we use 4 step Euler sampling for SDXL-Lightning and its LoRA variant, 4 step iterative random sampling for DMD2, LCM, and LCM-LoRA (incompatible with conventional solvers), and 4 step DPM++ 2S Ancestral sampling \cite{lu2022dpmpp} for SDXL-Turbo, utilizing DreamShaper \cite{dreamshaper2024}, an open-source customized model from the community. 

All quantitative results presented in the main paper are obtained using Algorithm 1, which employs a fully random renoising process (Line 12) to ensure generality. For distillation models that directly approximate the score function (e.g., SDXL-Lightning, SDXL-Turbo), the renoising strategy can be extended by incorporating the predicted epsilon from the previous time step. While the performance gains are marginal, we observed some improvement, likely due to adherence to the fundamental refinement principle of reverse diffusion sampling, as studied in \cite{kim2024dreamsampler}.

For all quantitative analyses, we fix the number of teacher guidance steps at $k=1$. Our approach remains simple with minimal hyperparameters, where the teacher guidance scale 
$\lambda$ is the primary parameter. Specifically, we set 
$\lambda=0.02$ for LCM, LCM-LoRA, and DMD2, and 
$\lambda=0.1$ for SDXL-Turbo, SDXL-Lightning, and SDXL-Lightning LoRA. The same $\lambda$ values are used in Fig. \ref{fig: teacher guidance} to evaluate the teacher guidance approximation.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.94\textwidth]{figure/tweedie_evolution.jpg}
    \caption{The evolution of denoised estimates differs between baseline (LCM-LoRA) and ours (8 total sampling steps). For the visualization, we decode $\tweedieppc(t)$ in Algorithm 1 to the pixel-space. Inferece-time distillation is applied only in the early sampling stage ($\text{Step}=8,7$).}
    \label{fig: tweedie}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.94\textwidth]{figure/teacher_compare.jpg}
    \caption{Comparisons between SDXL teacher model (8 steps) and ours. Our results are from the Fig. \ref{fig: result} of the main paper.}
    \label{fig: teacher compare}
\end{figure*}

\section{Additional results}
\label{sec: additional results}
In Fig \ref{fig: supple results 1} and \ref{fig: supple results 2}, we demonstrate the effectiveness of the proposed inference-time distillation with various student models. This advances stem from the guidance of teacher model, whereas the teacher model itself does not guarantee high-quality samples with few sampling steps, e.g. 8 steps (Fig \ref{fig: teacher compare}). That said, our work fosters a synergistic collaboration between two kinds of diffusion models: fast but sub-optimal student models, and high-quality buy computationally expensive teacher models.

Fig \ref{fig: tweedie} illustrates the evolution of the posterior mean through Tweedie’s formula \cite{efron2011tweedie} during the reverse diffusion process of student model and ours. Specifically, the intermediate estimates are decoded into the pixel space for visualization, and inference-time distillation is applied to the early sampling stage, i.e. $\text{Step}=8, 7$. We observe that the overall spatial layout of baseline (LCM-LoRA) is already defined in the early sampling stage, thereby disregarding the core concept, e.g. `old sea captain', in later sampling phase. In contrast, the inference-time distillation perturbs the initial student estimates by interpolating with teacher estimate, reflecting greater uncertainty about the spatial structure before the generation process unfolds further. This leads to the improved text-adherence as shown in the final outputs.

 

\section{Discussions and Limitations}
\label{sec: discussion}
Beyond the image domain, diffusion models have become a cornerstone of high-dimensional visual generative modeling, including applications such as video generation \cite{ho2022video} and multi-view synthesis \cite{voleti2025sv3d}. While computational efficiency is critical for modeling in these high-dimensional spaces, recent studies highlight the challenge of reducing inference steps for video generation. Compared to the image generation, the quality and prompt alignment of generated motion are more dependent on the number of inference steps \cite{polyak2024movie}. Although an increasing number of video diffusion distillation models \cite{zhai2024motion, lin2024animatediff} have emerged, a significant gap remains between student and teacher video diffusion models. Applying inference-time diffusion distillation to the video domain offers a promising avenue for improving temporal consistency, addressing issues that text-to-video (T2V) models--often adapted from text-to-image (T2I) models--frequently encounter.

Additionally, flow-based generative models generalize diffusion models and similarly rely on off-the-shelf ODE solvers. Thus, extending inference-time distillation to bridge the gap between flow-based teacher models (e.g., \cite{esser2024scaling}) and student models (e.g., \cite{sauer2024fast}) presents an intriguing direction for future research.

One limitation of the proposed framework is that both student and teacher (latent) diffusion models must operate within a shared latent space to enable interpolation between denoised estimates. To address this, one potential approach could involve mapping latent estimates back to pixel space, refining the student’s pixel estimates, and subsequently re-encoding them. Furthermore, the interplay between students and diverse open-source customized teacher models, which exhibit varying styles and aesthetics, represents another compelling avenue for exploration.


\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figure/supple_result.jpg}
    \caption{Qualitative comparisons against state-of-the-art distillation baselines. Baselines using 4 sampling steps: SDXL-Lightning, DMD2, SDXL-Turbo. Baselines using 8 sampling steps: LCM, LCM-LoRA.}
    \label{fig: supple results 1}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figure/supple_result2.jpg}
    \caption{Additional qualitative comparisons against state-of-the-art distillation baselines.}
    \label{fig: supple results 2}
\end{figure*}
